HumanEval-V: Benchmarking High-Level Visual Reasoning with Complex Diagrams in Coding Tasks

Understanding and reasoning over diagrams is a fundamental aspect of human intelligence. While Large Multimodal Models (LMMs) have demonstrated impressive capabilities across various tasks, existing benchmarks lack comprehensive evaluation of their diagram interpretation and reasoning abilities, particularly in coding contexts. We present HumanEval-V, a rigorous benchmark of human-annotated coding tasks that spans six task types and evaluates diverse visual reasoning capabilities. Each task features carefully crafted diagrams paired with function signatures and test cases, employing novel code generation tasks to thoroughly assess models' diagram comprehension. Through extensive experiments with 22 LMMs, we find that even top-performing models achieve modest success rates, with Claude 3.5 Sonnet reaching only 36.8% pass@1, highlighting substantial room for improvement. Our analysis reveals that current LMMs struggle with spatial transformations, topological relationships, and dynamic patterns that humans find intuitive. These findings provide valuable insights for advancing LMMs' visual reasoning abilities. We have open-sourced our code and benchmark at https://github.com/HumanEval-V/HumanEval-V-Benchmark.

==> tables_and_figures/related_work.tex <==
% \begin{table*}[ht]
% \centering
% \footnotesize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lllllll}
% \toprule
% \textbf{Benchmark} & \textbf{\# D.} & \textbf{Diagram Source} & \textbf{Task Source}  & \textbf{Task Type}  & \textbf{Evaluation Method} & \textbf{V.} \\
% \midrule
% \grayline \multicolumn{7}{c}{\textit{Benchmarks related to Scientific, Mathematical, or Analytical Diagrams}} \\
% AI2D~\cite{kembhavi2016diagram} & 5k & Crawled & Manually Created  & Multiple Choice & Exact Match with Ground Truth & \ding{56}   \\
% MM-Vet~\cite{yu2023mm} & 200*  & Crawled & Manually Created & Open-ended & LLM Scoring Based on Ground Truth & \ding{51}   \\
% MMBench~\cite{liu2023mmbench} & \textasciitilde3.2k*  & Crawled & Crawled & Multiple Choice & Exact Match with Ground Truth  & \ding{51}   \\
% MathVista~\cite{lu2023mathvista} & \textasciitilde6.1k* & Crawled & Crawled  & MCQ + Open-ended & Exact Match with Ground Truth & \ding{56}   \\
% MMMU~\cite{yue2024mmmu} & \textasciitilde11k* & Crawled & Crawled & Multiple Choice & Exact Match with Ground Truth & \ding{56}   \\
% Math-Vision~\cite{wang2024measuring} & \textasciitilde3k & Crawled & Crawled  & MCQ + Open-ended & Exact Match with Ground Truth  & \ding{56}   \\
% ChartQA~\cite{masry2022chartqa} & \textasciitilde1.6k  & Crawled & Manually Created  & Open-ended & Exact Match with Ground Truth  & \ding{56}   \\
% Charxiv~\cite{wang2024charxiv} & \textasciitilde2.3k  & Crawled & Manually Created & Open-ended & Exact Match with Ground Truth  & \ding{51}   \\
% Chartmimic~\cite{shi2024chartmimic}  & 500  & Manually Created & Manually Created & Code Generation & LLM Scoring + Rule-based Similarity & \ding{51}   \\
% \midrule
% \grayline \multicolumn{7}{c}{\textit{Benchmarks related to Visual Abstract Reasoning Diagrams}} \\
% RAVEN~\cite{zhang2019raven}  & \textasciitilde22k  & Auto-generated & Auto-generated & Multiple Choice & Exact Match with Ground Truth  & \ding{51}   \\
% ARC-AGI~\cite{chollet2019measure}  & 400     & Auto-generated & Auto-generated & Matrix Generation & Exact Match with Ground Truth  & \ding{51}   \\
% Bongard~\cite{nie2020bongard} & 1.8k    & Auto-generated & Auto-generated  & Binary Choice & Exact Match with Ground Truth  & \ding{51}   \\
% MARVEL~\cite{jiang2024marvel}  & 770  & Crawl + Manual & Crawl + Manual & Multiple Choice & Exact Match with Ground Truth & \ding{51}   \\
% \midrule
% \grayline \multicolumn{7}{c}{\textit{Benchmarks related to Programmatic Abstract Diagrams}} \\
% MMCode~\cite{li2024mmcode} & \textasciitilde3.5k*  & Crawled & Crawled  & Code Generation & Pass Rate based on Test Cases & \ding{56}  \\
% HumanEval-V (Ours) & 253  & Manually Created & Manually Created  & Coding or Description & Pass Rate based on Test Cases & \ding{51}   \\
% \bottomrule
% \end{tabular}
% }
% \caption{A comparison of HumanEval-V to other diagram-related benchmarks. \textbf{\# D.} indicates the number of unique diagrams in the test set. \textbf{V.} denotes whether visual information is necessary for solving all tasks (\ding{51}) or not (\ding{56}). An asterisk (*) means the actual number of diagrams is lower than the given count due to the inclusion of natural or other non-diagram images.}
% \label{tab:benchmarks}
% \end{table*}
